A Nonlinear Singular Value Theory for Neural Networks

Recently Brown et al. [2025] established a singular value decomposition (SVD) for maps (especially nonlinear) satisfying certain norm conditions. We prove that most modern neural architectures admit this nonlinear SVD (NLSVD) representation---with no change in input--output behavior---and enumerate the classes covered. In this factorization the network is a left-invertible nonlinear map followed by a final linear layer. Moreover, the left-invertible factor is norm-preserving, so distances in the embedding (activations before the final linear layer) calibrate directly to distances in input space. We introduce a flexible architecture that yields an explicit decomposition at training time, a data-driven algorithm for estimating the representation from trained models, and the mathematical foundations for nonlinear analogues of row and null spaces in neural networks. Empirical case studies illustrate uses of the theory for latent-space pullback (visualization and data generation), bias detection, and membership-inference robustness under training. Altogether, these foundations support new approaches to core problems in neural-network analysis.

==> 89-required-stuff.tex <==
\paragraph{Software and Data.}
For review, code has been uploaded as supplementary material and will be made
available as a live GitHub link following publication.

\paragraph{Impact Statement.}
This paper advances basic machine-learning research.  The framework may support
algorithmic development and understanding of nonlinear functions, especially
neural networks.  As our results illustrate, techniques stemming from this work
may also identify, exacerbate, or help remediate AI-security issues.

% Acknowledgments are intentionally omitted from the anonymous review paper.
% The funding statement is preserved in camera-ready-acknowledgments.tex.


==> collaborator_review/revision_blocks/20-architecture-brian.tex <==
The same argument covers stateful transformers over a fixed finite horizon when the carried state is finite-dimensional and restricted to a compact domain, since the state is included in the input and output of each update map. However, it does not provide a uniform finite-gain bound for unbounded state or arbitrarily long iteration.

\begin{center}
\fbox{%
\begin{minipage}{0.94\columnwidth}
\footnotesize
\textbf{NLSVD coverage for modern neural networks.}
After anchoring at a reference input, the following architectures have finite
\(2\)-induced gain and therefore admit an NLSVD under the stated
restrictions.

\medskip
\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}p{0.42\linewidth}>{\raggedright\arraybackslash}X@{}}
\textbf{Architecture} & \textbf{Required restriction} \\
\hline
MLPs, CNNs, ResNets, and U-Nets
  & Finite composition on a compact input domain \\
RNNs and recurrent networks
  & Finite horizon and compact hidden-state domain \\
Fixed-length transformers
  & Compact token domain and fixed attention mask \\
Encoder--decoder transformers
  & Bounded source and target lengths \\
Stateful transformers
  & Finite-dimensional compact state and finite update horizon \\
Diffusion U-Net denoisers
  & Fixed time and conditioning, with deterministic evaluation
\end{tabularx}

\medskip
Unbounded attention inputs, unbounded carried state, and arbitrarily long
iteration are not covered. The formal result and proof appear in
Theorem~\ref{thm:architecture} of the supplement.
\end{minipage}}
\end{center}


==> collaborator_review/revision_blocks/20-architecture-original.tex <==
\todo{does this apply to statefull transformers?}
\todo{add a table or bullet list of architectures this applies to}
\todo{potentially replace this theorem with ``the following architectures satisfy the 2-induced norm property''}
\begin{theorem}[Modern architectures give anchored finite-gain maps]
\label{thm:architecture}
Let \(\X_0\) be compact, let \(T<\infty\), and for \(t=1,\ldots,T\) let
\(H_t:\X_{t-1}\to\X_t\) be blocks with \(\X_t=H_t(\X_{t-1})\).
Define the realized map by \(f=H_T\circ\cdots\circ H_1:\X_0\to\X_T\).
Suppose each block \(H_t\) is one
of the affine, convolutional, pooling/downsampling, coordinatewise-activation,
stabilized-normalization, residual, concatenation, feedforward, self-attention,
masked-attention, or encoder--decoder cross-attention blocks covered by Appendix
Lemma~\ref{lem:lipschitz-calculus}, the fixed-length attention
bound of ~\cite{castin2024smoothattention}, and Lemma~\ref{lem:cross-attention-lipschitz}.
For fixed finite token dimensions and fixed attention masks, let \(L_t<\infty\) be a Lipschitz constant for \(H_t\) on \(\X_{t-1}\).
Then \(\mathrm{Lip}(f;\X_0)\le \prod_{t=1}^T L_t < \infty\).
%the \(t\)-th block's Lipschitz constant. Then \(\mathrm{Lip}(f;\X_0)\le \prod_{t=1}^T L_t < \infty\).
Consequently, for any fixed-length token domain anchor \(x_\star\in\X_0\), the recentered deviation map
\(f_\star(h)=f(x_\star+h)-f(x_\star)\) has finite induced gain by
Theorem~\ref{thm:compact-bound}.  If only finitely many source/target sequence
lengths are allowed, the family constant is
\(\max_{(n_s,n_t)}\prod_t L_{t,n_s,n_t}<\infty\). \quad \noindent\textit{Proof.} See Appendix~\ref{app:modern-architecture-proofs}.
\end{theorem}


==> collaborator_review/revision_blocks/20-architecture-priority.tex <==
\begin{theorem}[Modern architectures give anchored finite-gain maps]
\label{thm:architecture}
Let \(\X_0\) be compact, let \(T<\infty\), and for \(t=1,\ldots,T\) let
\(H_t:\X_{t-1}\to\X_t\) be blocks with \(\X_t=H_t(\X_{t-1})\).
Define the realized map by \(f=H_T\circ\cdots\circ H_1:\X_0\to\X_T\).
Suppose each block \(H_t\) is one
of the affine, convolutional, pooling/downsampling, coordinatewise-activation,
stabilized-normalization, residual, concatenation, feedforward, self-attention,
masked-attention, or encoder--decoder cross-attention blocks covered by Appendix
Lemma~\ref{lem:lipschitz-calculus}, the fixed-length attention
bound of ~\cite{castin2024smoothattention}, and Lemma~\ref{lem:cross-attention-lipschitz}.
For fixed finite token dimensions and fixed attention masks, let \(L_t<\infty\) be a Lipschitz constant for \(H_t\) on \(\X_{t-1}\).
Then \(\mathrm{Lip}(f;\X_0)\le \prod_{t=1}^T L_t < \infty\).
Consequently, for any fixed-length token domain anchor \(x_\star\in\X_0\), the recentered deviation map
\(f_\star(h)=f(x_\star+h)-f(x_\star)\) has finite induced gain by
Theorem~\ref{thm:compact-bound}.  If only finitely many source/target sequence
lengths are allowed, the family constant is
\(\max_{(n_s,n_t)}\prod_t L_{t,n_s,n_t}<\infty\). \quad \noindent\textit{Proof.} See Appendix~\ref{app:modern-architecture-proofs}.
\end{theorem}


==> collaborator_review/revision_blocks/51-radial-calibration-brian.tex <==
% SUPERSEDED: content lives in 52-nlsvd-vs-ae.tex (input from main.tex).
% Do not \input or RevisionAddInput this file in main/main-clean/main-marked builds.
We isolate the decoder calibration used by these traversals by training an NLSVDNet and an architecture-matched autoencoder on MNIST. The models each contain \(1{,}622{,}809\) trainable parameters, begin from identical weights, receive the same minibatches, and attain held-out accuracies of \(97.45\%\) and \(97.55\%\), respectively. Figure~\ref{fig:radial-distance-row-null} compares latent radius with the radius of the raw decoded output after moving through the row and null spaces of the final linear layer. The mean relative radial error for NLSVDNet is \(4.13\times10^{-8}\) in the row space and \(4.50\times10^{-8}\) in the null space, compared with \(0.621\) and \(0.572\) for the matched autoencoder. The measurement uses radius from the zero input. Pairwise distance, traversal length, and arc length remain outside its scope. The result establishes radial calibration of the ambient decoder without asserting that the sampled latent points lie on the learned encoder image.



==> collaborator_review/revision_blocks/90-architecture-theorem-brian.tex <==
\begin{theorem}[Modern architectures give anchored finite-gain maps]
\label{thm:architecture}
Let \(\X_0\) be compact, let \(T<\infty\), and for \(t=1,\ldots,T\) let
\(H_t:\X_{t-1}\to\X_t\) be blocks with \(\X_t=H_t(\X_{t-1})\).
Define the realized map by \(f=H_T\circ\cdots\circ H_1:\X_0\to\X_T\).
Suppose each block \(H_t\) is one
of the affine, convolutional, pooling/downsampling, coordinatewise-activation,
stabilized-normalization, residual, concatenation, feedforward, self-attention,
masked-attention, or encoder--decoder cross-attention blocks covered by
Lemma~\ref{lem:lipschitz-calculus}, the fixed-length attention
bound of ~\cite{castin2024smoothattention}, and Lemma~\ref{lem:cross-attention-lipschitz}.
For fixed finite token dimensions and fixed attention masks, let \(L_t<\infty\) be a Lipschitz constant for \(H_t\) on \(\X_{t-1}\).
Then \(\mathrm{Lip}_{\X_0}(f)\le \prod_{t=1}^T L_t < \infty\).
Consequently, for any fixed-length token domain anchor \(x_\star\in\X_0\), the recentered deviation map
\(f_\star(h)=f(x_\star+h)-f(x_\star)\) has finite induced gain by
Theorem~\ref{thm:compact-bound}. If only finitely many source/target sequence
lengths are allowed, the family constant is
\(\max_{(n_s,n_t)}\prod_t L_{t,n_s,n_t}<\infty\).
\end{theorem}

